Assessing and improving reliability of neighbor embedding methods: a map-continuity perspective

Visualizing high-dimensional data is essential for understanding biomedical data and deep learning models. Neighbor embedding methods, such as t-SNE and UMAP, are widely used but can introduce misleading visual artifacts. We find that the manifold learning interpretations from many prior works are inaccurate and that the misuse stems from a lack of data-independent notions of embedding maps, which project high-dimensional data into a lower-dimensional space. Leveraging the leave-one-out principle, we introduce LOO-map, a framework that extends embedding maps beyond discrete points to the entire input space. We identify two forms of map discontinuity that distort visualizations: one exaggerates cluster separation and the other creates spurious local structures. As a remedy, we develop two types of point-wise diagnostic scores to detect unreliable embedding points and improve hyperparameter selection, which are validated on datasets from computer vision and single-cell omics.

==> tex_files/TableForDatasetOverview_backup.tex <==
\begin{table}[h]
\footnotesize
\centering
\begin{tabular}{ccccc}
\hline
Dataset                     &Points & Dimensions & Domain  & Usage      \\ \hline
CIFAR-10 \cite{KrizhevskyCIFAR102009}                          &  10,000  &   512               & Deep learning& Perturbation score, verification of LOO assumption \\
DTD \cite{CimpoiDTD2014}         &  5,640      &   512            & Deep learning& Perturbation score (OOD detection)\\
Embryo \cite{HayashiData}&  421       &  2,000              & Single-cell &                 Singularity score\\
Brain \cite{luecken}          &  3,618    &  1,000               & Single-cell&   Singularity score, verification of LOO assumption               \\
IFNB \cite{ifnb}                          &  6,548      &  2,000             & Single-cell &   Verification of LOO assumption              \\
Panc8 \cite{panc8}                  &  2,364        &   2,000          & Single-cell  &    Verification of LOO assumption      \\      
Mammary \cite{Bach2017MammaryData}     &  25,806        &   2,000          & Single-cell  &   Singularity score            \\ 
\hline
\end{tabular}
\caption{\textbf{Datasets analyzed in this work.} This paper analyzes seven real-world datasets: CIFAR-10, Describable Textures Dataset (DTD), the mouse embryonic stem cell differentiation data (Embryo), the single-cell RNA-seq dataset generated from PBMCs treated with interferon-$\beta$ (IFNB),  the mouse brain single-cell ATAC-seq data (Brain), the single-cell RNA-seq dataset generated from human pancreatic tissues (Panc8), the single-cell dataset of mammary epithelial cells (Mammary). The table lists the number of points, dimensions, domains, and usage of the datasets.}  
\label{tab: datasetoverview}
\end{table}

==> tex_files/TableForMouseBrainTests_copy.tex <==

\renewcommand{\arraystretch}{1.2}

\begin{table}[htbp]
\footnotesize
\centering
\begin{subtable}[h]{\textwidth}
\centering
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{l|}{}                                                                                                  & \multicolumn{1}{c|}{}        & \multicolumn{2}{c|}{Perplexity 4}                                       & \multicolumn{2}{c}{Perplexity 25}                            \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Test for\\ Spearman's\\ Rank Correlation\end{tabular}}} & \multicolumn{1}{c|}{Class}   & \multicolumn{1}{c|}{$p$-value}  & \multicolumn{1}{c|}{Corrected $p$-value*} & \multicolumn{1}{c|}{$p$-value}            & Corrected $p$-value* \\ \cline{2-6} 
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{1}       & \multicolumn{1}{c|}{$0.0757$} & \multicolumn{1}{c|}{$0.3026$}           & \multicolumn{1}{c|}{$0.0000$}           & $0.0000$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{2}       & \multicolumn{1}{c|}{$0.1298$} & \multicolumn{1}{c|}{$0.3895$}           & \multicolumn{1}{c|}{$6.3\times10^{-5}$} & $1.9\times10^{-4}$ \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{3}       & \multicolumn{1}{c|}{$0.0389$} & \multicolumn{1}{c|}{$0.1945$}           & \multicolumn{1}{c|}{$2.7\times10^{-5}$} & $1.1\times10^{-4}$ \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{4}       & \multicolumn{1}{c|}{$0.2493$} & \multicolumn{1}{c|}{$0.4533$}           & \multicolumn{1}{c|}{$0.7408$}           & $0.7408$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{5}       & \multicolumn{1}{c|}{$0.2266$} & \multicolumn{1}{c|}{$0.4533$}           & \multicolumn{1}{c|}{$4.0\times10^{-3}$} & $8.0\times10^{-3}$           \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}F-test for\\ Local Regression Model\end{tabular}}                       & \multicolumn{1}{l|}{$p$-value} & \multicolumn{2}{c|}{$0.3598$}                                           & \multicolumn{2}{c}{$9.7\times10^{-4}$}                     \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Permutation Test for\\ Local Regression Model\end{tabular}}             & \multicolumn{1}{c|}{$p$-value} & \multicolumn{2}{c|}{$0.3195$}                                           & \multicolumn{2}{c}{$0.0074$}                                 \\ \hline
\multicolumn{6}{l}{* Use Holm-Bonferroni correction for multiple testing.}           
\end{tabular}
\caption{Tests of singularity score pattern in single-cell RNA-seq data of mouse embryonic stem cells differentiation.}
\end{subtable}
\hfill
\vspace{0.5cm}
\begin{subtable}[h]{\textwidth}
\centering
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{}                   & \multicolumn{2}{c|}{Perplexity 5}                                       & \multicolumn{2}{c}{Perplexity 95}                            \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Test for\\ Spearman's\\ Rank Correlation\end{tabular}}} & \multicolumn{1}{c|}{Class}              & \multicolumn{1}{c|}{$p$-value}  & \multicolumn{1}{c|}{Corrected $p$-value*} & \multicolumn{1}{c|}{$p$-value}            & Corrected $p$-value* \\ \cline{2-6} 
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{Astrocytes}         & \multicolumn{1}{c|}{$0.2136$} & \multicolumn{1}{c|}{$1.0000$}           & \multicolumn{1}{c|}{$0.5048$}           & $0.5048$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{Endothelial Cells}  & \multicolumn{1}{c|}{$0.5594$} & \multicolumn{1}{c|}{$1.0000$}           & \multicolumn{1}{c|}{$0.0651$}           & $0.1893$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{Excitatory Neurons} & \multicolumn{1}{c|}{$0.7461$} & \multicolumn{1}{c|}{$1.0000$}           & \multicolumn{1}{c|}{$1.2\times10^{-5}$} & $5.9\times10^{-5}$ \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{Inhibitory Neurons} & \multicolumn{1}{c|}{$0.0470$} & \multicolumn{1}{c|}{$0.2820$}           & \multicolumn{1}{c|}{$0.0631$}           & $0.1893$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{Microglia}          & \multicolumn{1}{c|}{$0.3735$} & \multicolumn{1}{c|}{$1.0000$}           & \multicolumn{1}{c|}{$1.2\times10^{-7}$} & $7.3\times10^{-7}$ \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{Oligodendrocytes}   & \multicolumn{1}{c|}{$0.6364$} & \multicolumn{1}{c|}{$1.0000$}           & \multicolumn{1}{c|}{$3.9\times10^{-3}$} & $0.0156$           \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}F-test for\\ Local Regression Model\end{tabular}}                       & \multicolumn{1}{c|}{$p$-value}            & \multicolumn{2}{c|}{$0.1013$}                                          & \multicolumn{2}{c}{$<2.2\times10^{-16}$}                     \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Permutation Test for\\ Local Regression Model\end{tabular}}             & \multicolumn{1}{c|}{$p$-value}            & \multicolumn{2}{c|}{$0.0610$}                                           & \multicolumn{2}{c}{$0.0000$}                                 \\ \hline
\multicolumn{6}{l}{* Use Holm-Bonferroni correction for multiple testing.}  
\end{tabular}
\caption{Tests of singularity score pattern in mouse brain single-cell ATAC-seq data.}
\end{subtable}
\hfill
\vspace{0.5cm}
\begin{subtable}[h]{\textwidth}
\centering
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{}                   & \multicolumn{2}{c|}{Perplexity 30}                                       & \multicolumn{2}{c}{Perplexity 175}                            \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Test for\\ Spearman's\\ Rank Correlation\end{tabular}}} & \multicolumn{1}{c|}{Class}              & \multicolumn{1}{c|}{$p$-value}  & \multicolumn{1}{c|}{Corrected $p$-value*} & \multicolumn{1}{c|}{$p$-value}            & Corrected $p$-value* \\ \cline{2-6} 
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{NP1}         & \multicolumn{1}{c|}{$0.9962$} & \multicolumn{1}{c|}{$1.0000$}           & \multicolumn{1}{c|}{$0.3623$}           & $1.0000$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{NP2}  & \multicolumn{1}{c|}{$0.0557$} & \multicolumn{1}{c|}{$0.2223$}           & \multicolumn{1}{c|}{$0.4702$}           & $1.0000$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{G1}  & \multicolumn{1}{c|}{$0.6469$} & \multicolumn{1}{c|}{$1.0000$}           & \multicolumn{1}{c|}{$7.1\times10^{-14}$}           & $3.5\times10^{-13}$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{G2}  & \multicolumn{1}{c|}{$0.0147$} & \multicolumn{1}{c|}{$0.0734$}           & \multicolumn{1}{c|}{$1.1\times10^{-15}$}           & $6.8\times10^{-15}$           \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{L1} & \multicolumn{1}{c|}{$2.7\times10^{-25}$} & \multicolumn{1}{c|}{$2.2\times10^{-24}$}           & \multicolumn{1}{c|}{$3.3\times10^{-150}$} & $2.6\times10^{-149}$ \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{L2}          & \multicolumn{1}{c|}{$1.5\times 10^{-8}$} & \multicolumn{1}{c|}{$1.1\times 10^{-7}$}           & \multicolumn{1}{c|}{$5.2\times10^{-76}$} & $3.6\times 10^{-75}$ \\
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{PI1}          & \multicolumn{1}{c|}{$0.5188$} & \multicolumn{1}{c|}{$1.0000$}           & \multicolumn{1}{c|}{$0.8746$} & $1.0000$ \\ 
\multicolumn{1}{c|}{}                                                                                                  & \multicolumn{1}{c|}{PI2}   & \multicolumn{1}{c|}{$0.0022$} & \multicolumn{1}{c|}{$0.0131$}           & \multicolumn{1}{c|}{$4.6\times 10^{-11}$} & $1.8\times 10^{-10}$           \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}F-test for\\ Local Regression Model\end{tabular}}                       & \multicolumn{1}{c|}{$p$-value}            & \multicolumn{2}{c|}{$0.2979$}                                          & \multicolumn{2}{c}{$5.3\times10^{-14}$}                     \\ \hline
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Permutation Test for\\ Local Regression Model\end{tabular}}             & \multicolumn{1}{c|}{$p$-value}            & \multicolumn{2}{c|}{$0.2379$}                                           & \multicolumn{2}{c}{$0.0000$}                                 \\ \hline
\multicolumn{6}{l}{* Use Holm-Bonferroni correction for multiple testing.}  
\end{tabular}
\caption{Tests of singularity score pattern in mammary epithelial cell dataset.}
\end{subtable}

\caption{\textbf{Tests of the distribution difference of singularity scores in (a) mouse embryonic stem cell differentiation data and (b) mouse brain chromatin accessibility data.} We verifiy the distribution difference using Spearman’s rank correlation tests between singularity scores and distances to cluster centers, F-tests and per- mutation tests for a local regression model (singularity scores regressed against locations). The results of all three tests confirm the distribution difference of singularity scores between small and large perplexities.}  
\label{tab: mousebraintest}
\end{table}

==> tex_files/interpolation-property.tex <==
\begin{prop}
Given $\mX = [\vx_1, \ldots, \vx_n]^\top$ and their corresponding embedding points $\mY = [\vy_1, \ldots, \vy_n]^\top$, under the LOO assumption, the LOO-map $\tilde{f}$ induced by $\mX$ and $\mY$ exhibits the interpolation property such that 
$$
\tilde{f}(\vx_i) \approx \vy_i,\quad i = 1, \ldots, n.
$$
\label{thm: prop1}
\end{prop}

==> tex_files/introduction.tex <==

% \TODO{Inconsistent reference to sections and appendix: Sec. or Section, Supplemental file or Supplemental etc.}

% \TODO{Inconsistent naming, e.g., sub-cluster vs.~subcluster.}
\hengheng{The introduction part is too long for this type of paper. Now 1,100 words, while 541 words in DynamicViz, and 761 words in scDEED. Need to revise later.}

Data visualization plays a crucial role in modern data science, as it offers essential and intuitive insights into high-dimensional datasets by providing low-dimensional embeddings of the data. Classical methods for dimension reduction include principal component analysis (PCA) \cite{kppca1901}, multidimensional scaling \cite{TorgersonMDS1952}, locally linear embedding \cite{RoweisLLE2000}, among others.
For visualizing high-dimensional data, the last two decades have witnessed rising popularity of 
t-SNE \cite{HintonTSNE2008} and UMAP \cite{mcinnesUMAP2018}, which are extensively used in, e.g., single-cell analysis \cite{kobak2019art,linderman2019fast,luecken2019current} and feature interpretations for deep learning models \cite{JING2022LayerUMAP,Islam2023DNNManifoldLearning}. 

%The stochastic neighbor embedding methods are a family of visualization methods---including t-SNE, UMAP, and LargeVis among others---which determine embedding points directly by a complicated optimization algorithm \Rong{please be more specific: good to mention that each of these methods minimizes some kind of  discrepancy between the similarity measures in high-D input data and their low-D embedding points}: given input points $\vx_1,\ldots,\vx_n$, an algorithm $\gA$ finds embedding \Rong{note that the ``embedding" here is defined by the aforementioned discrepancy minimizing algorithm, not a mathematically rigorous embedding. Good to convey this point somehow through our narrative.} points $(\vy_1, \ldots, \vy_n) = \gA(\vx_1,\ldots,\vx_n)$ in the 2D plane. This approach is very different from classical dimension reduction methods such as PCA, where a parametric mapping $\vf_{\vtheta}$ is determined and any input point $\vx$ is embedded through $\vy = \vf_{\vtheta}(\vx)$. 

 The neighbor embedding methods \cite{probabilistic_view_of_NE, BoydMDE2021} are a family of visualization methods, which include t-SNE, UMAP, and LargeVis \cite{largevis} as popular examples, that determine embedding points directly by solving a complicated optimization algorithm to minimize the discrepancy between similarities of input data points and those of the corresponding low-dimensional points.  Given input data $\vx_1,\ldots,\vx_n$, a neighbor embedding algorithm $\gA$ computes the points $(\vy_1, \ldots, \vy_n) = \gA(\vx_1,\ldots,\vx_n)$ in the 2D plane, aiming to preserve the essential structures of $\vx_1,\ldots,\vx_n$. Due to the algorithmic complexity, $\gA$ is often used as a black-box visualization tool. This is very different from classical dimension reduction methods such as PCA, where a parametric mapping $\vf_{\vtheta}$ is determined and any input point $\vx$ is embedded through $\vy = \vf_{\vtheta}(\vx)$. For neighbor embedding methods, in contrast, there is no clearly defined embedding map for the ``embedding points'' $\vy_1, \ldots, \vy_n$.


Due to the lack of explicit embedding maps \cite{AuffingerEquilibriumDistributionsTDistributedStochastic2023}, neighbor embedding methods suffer from both conceptual and practical difficulties. For conceptual difficulties, there is no obvious sample-independent notion of embedding maps, since the embedding points $\vy_1,\ldots, \vy_n$ depend on $n$ input points $\vx_1,\ldots, \vx_n$ collectively, which makes it challenging to understand the correspondence between an input point $\vx_i$ and an embedding point $\vy_i$. Thus, it is unclear what structures the embedding points inherit from the input points, even in ideal settings where inputs are drawn from known distributions or simple manifolds.

For practical difficulties, it has been recently recognized that neighbor embedding methods often produce misleading results by creating severe distortion through the embedding maps and introducing spurious clusters in low-dimensional visualization \cite{WangPacMap2021, ChariSpeciousArt2023}. Moreover, neighbor embedding methods are sensitive to the choice of optimization algorithms \cite{YangOptimizationTSNE2015}, initialization schemes \cite{KobakInitializationImportantForTSNEUMAP2019},
%initialization \cite{KobakInitializationImportantForTSNEUMAP2019}, optimization algorithms \cite{YangOptimizationTSNE2015}
and hyperparameters \cite{KobakInitializationImportantForTSNEUMAP2019,Ma2022theoreticalfoundationoft-SNE}, which may lead to inconsistent interpretations \cite{AllOfUs2024}. 

Some progress has been made, but significant challenges remain. On the theoretical side, insights have been obtained regarding embedding stages \cite{Ma2022theoreticalfoundationoft-SNE,arora2018analysistsnealgorithmdata,linderman2019Clusteringwitht-SNEProvably}, force-based interpretations \cite{steinerberger2022t-SNEforcefulcolorings},  and visualization quality \cite{arora2018analysistsnealgorithmdata,linderman2019Clusteringwitht-SNEProvably,shaham2017stochasticneighborembeddingseparates}.
%\cite{auffinger2023equilibriumdistributionstdistributedstochastic} \TODO{find refs} provide insights into the optimization algorithms and blabla. 
On the practical side, schemes of robust initialization and hyperparameter selection have been proposed \cite{kobak2019art,ChariSpeciousArt2023, wattenberg2016how,  BelkinaAutoOptParaTSNE2019, scDEED2023}. To enhance the faithfulness of neighbor embedding methods, multiple diagnostic quantities have been proposed \cite{kobak2019art,ChariSpeciousArt2023, wattenberg2016how,  BelkinaAutoOptParaTSNE2019}. In particular, Johnson et~al.~\cite{EMBEDR} and Xia et~al.~\cite{scDEED2023} propose algorithms to detect embedding points with severe neighborhood distortion, whereas Sun et~al.~\cite{dynamicviz} propose a dynamic approach to assess visualization uncertainty. However, due to a limited understanding of the origins and nature of the observed artifacts, most existing diagnostic methods offer only partial solutions and rely on ad hoc fixes, sometimes even introducing new artifacts (Figure~\ref{fig: methods-compare}).


%In this work, we address these difficulties by using a classical strategy from statistics known as the leave-one-out (LOO) method, which posits that adding, deleting, or changing a single input point has negligible effects on the overall inferential results. Using LOO, we may decouple one embedding point (say $\vy_n$) from the remaining ones: freezing $\vx_1,\ldots, \vx_{n-1}$ and $\vy_1,\ldots, \vy_{n-1}$, we have approximation $(\vy_1,\ldots, \vy_{n-1}, \vf_n(\vx)) \approx \gA(\vx_1,\ldots, \vx_{n-1}, \vx)$ in a neighborhood of $\vx = \vx_n$. We call $\vf_n(\vx)$ the \textit{implicit embedding map} \change{suggested name: LOO-map}, which maps a single input point to a single embedding point.
%as the \textit{implicit embedding map} defined in a neighborhood of $\vx = \vx_n$. 
%This approach allows us to view stochastic neighbor embedding methods as embedding maps in the classical sense: we may assess whether $\gA$ faithfully preserves underlying structures of input points such as clusters or manifolds by analyzing the map $\vf_n(\vx)$.\Rong{good to clarify how do we know if $\vf_n(\vx)$ is representative of the whole map? I think we essentially assume the input data has some underlying structure of interest, and the data points are random samples from certain underlying distribution. It is in this sense choosing any single point from the data can provide a view of the complete embedding landscape. -- need to better think about how to explain this point.}

In this work, we propose a notion of embedding map---which we call LOO-map---induced by a given neighbor embedding method $\gA$. LOO-map is a mapping in the classical sense and approximates the properties of $\gA$ around each embedding point. It is based on a classical strategy from statistics known as the leave-one-out (LOO) method, which posits that adding, deleting, or changing a single input point has negligible effects on the overall inferential results. 
%Using LOO, we may decouple one embedding point (say $\vy_n$) from the remaining ones: freezing $\vx_1,\ldots, \vx_{n-1}$ and $\vy_1,\ldots, \vy_{n-1}$, we have approximation $(\vy_1,\ldots, \vy_{n-1}, \vf(\vx)) \approx \gA(\vx_1,\ldots, \vx_{n-1}, \vx)$ in a neighborhood of $\vx = \vx_n$. 
Using LOO, we can decouple the pairwise interaction in the algorithm $\gA$: we add a new input point $\vx$ to $\vx_1,\ldots, \vx_{n}$ and freeze $\vy_1,\ldots, \vy_{n}$ in the optimization problem, allowing only one free variable $\vy$. We call the resulting minimizer $\vf(\vx)$ the LOO-map, which satisfies the approximation $(\vy_1,\ldots, \vy_{n}, \vf(\vx)) \approx \gA(\vx_1,\ldots, \vx_{n}, \vx)$. By design, the LOO-map $\vf$ not only satisfies $\vf(\vx_i) \approx \vy_i$ for all $i$'s, but also reveals the  embedding point $\vf(\vx)$ of a potential new input point $\vx$. As such, LOO-map extends the mapping defined over the discrete input set $\{\vx_1, \ldots, \vx_n\}$ to the entire input space.
%which yields the minimizer $\vf(\vx)$ that we we denote by $\vf(\vx)$. By LOO, we have approximation $(\vy_1,\ldots, \vy_{n}, \vf(\vx)) \approx \gA(\vx_1,\ldots, \vx_{n}, \vx)$.
%Using LOO, we may decouple a new input point $\vx$ from existing ones: freezing $\vx_1,\ldots, \vx_{n}$ and $\vy_1,\ldots, \vy_{n}$, we have approximation $(\vy_1,\ldots, \vy_{n}, \vf(\vx)) \approx \gA(\vx_1,\ldots, \vx_{n}, \vx)$. At each input point $\vx_i$, we have $\vf(\vx_i)$ This idea allows us to define a mapping around a neighborhood of each input point, which yields the LOO-map $\vf(\vx)$ defined in the input space. 
%LOO-map allows us to  assess stochastic neighbor embedding methods rigorously: we may assess whether $\gA$ faithfully preserves underlying structures of input points such as clusters or manifolds by analyzing the map $\vf(\vx)$.

% \hengheng{a rewrite of the last paragraph, but not good, please delete at your will}\hengheng{one struggle I have when trying to revise this paragraph is about the intuition of adding one point to the original dataset. Perturbing one existing point is natural. But adding one point is more vague.} In this work, we propose a notion of embedding map---which we call LOO-map---induced by a given stochastic neighbor embedding method $\gA$. LOO-map is a mapping in the classical sense and approximates the properties of $\gA$ \change{in the entire embedding space}. It is based on a classical strategy from statistics known as the leave-one-out (LOO) method, which posits that adding, deleting, or changing a single input point has negligible effects on the overall inferential results. Using LOO, we may \change{add one data point $\vx$ and study its embedding point (say $\vy$)} without rerunning : freezing \change{$\vx_1,\ldots, \vx_{n}$ and $\vy_1,\ldots, \vy_{n}$}, we have approximation \change{$(\vy_1,\ldots, \vy_{n}, \vf(\vx)) \approx \gA(\vx_1,\ldots, \vx_{n}, \vx)$}. This idea allows us to define a mapping around a neighborhood of each input point, which yields the LOO-map $\vf(\vx)$ defined in the input space. LOO-map allows us to 
% %view stochastic neighbor embedding methods as embedding maps in the classical sense: 
% assess stochastic neighbor embedding methods rigorously: we may assess whether $\gA$ faithfully preserves underlying structures of input points such as clusters or manifolds by analyzing the map $\vf(\vx)$.

LOO-map provides a unified framework for both understanding recognized issues such as distance distortion \cite{ChariSpeciousArt2023,globaltsne}, low stability \cite{dynamicviz}, and lack of neighborhood preservation \cite{ChariSpeciousArt2023, Cooley689851}, and uncovering novel insights such as embedding discontinuity. In our view, discontinuities of $\vf(\vx)$ represent an extreme form of distortion that accompanies topological changes in the embedding space, e.g., connected clusters become separated and a uniform shape is broken into fractured pieces. In contrast, classical dimension reduction methods such as PCA do not suffer from map discontinuity since a continuous parametric map $\vf_{\theta}(\vx)$ is constructed explicitly. In this regard, embedding discontinuity is an innate issue of the family of neighbor embedding methods.

Using LOO-map, we identify two types of observed distortion patterns, one affecting global properties of the embedding map and the other affecting local relationships. Both types of distortions are a consequence of discontinuities in $\vf(\vx)$ and can cause topological changes of the  embedding structures.

%that the recognized artifacts of stochastic neighbor embedding methods---such as embedding distortion and lack or robustness---are in fact a consequence of inherent discontinuity of the implicit embedding maps. We identify the following two types of observed discontinuity patterns, and trace their roots to the geometric properties of the implicit embedding map.


\begin{itemize}
    \item \textbf{Overconfidence-inducing (OI) discontinuity}. Overlapping clusters or data mixtures in the input space are embedded into well-separated clusters, which creates a misleading visual impression of over-confidence that there is less uncertainty in the datasets.
    This biased perception of uncertainty can, in turn, lead to overly confident scientific conclusions. %Consequently, an insufficient perception of uncertainty may lead to overconfident scientific conclusions. 
    \item \textbf{Fracture-inducing (FI) discontinuity}. Small spurious and artificial clusters form in the embedding space, even for non-clustered data. 
    %Unlike OI discontinuity, such spurious clusters are forms in arbitrary locations and vary across different random seeds. \TODO{We did not do subsampling, did we?} \hengheng{No} %vary in locations under subsampling of input data.
    Unlike OI discontinuity, such spurious clusters are small, localized, and formed in arbitrary locations. 

\end{itemize}
We propose two point-wise diagnostic scores, namely \textit{perturbation scores} and \textit{singularity scores}, to quantify the severity of the two types of map discontinuity at each embedding point. Our approach is flexible and works as a wrapper around many neighbor embedding algorithms (Supplementary File Section~\ref{sec: appendix: derivation of sscore})  without requiring any label information. To illustrate the diagnostic scores, we provide two use cases: the first shows that perturbation scores detect out-of-distribution data (or data with distribution shift) in computer vision, and the second shows that singularity scores aid users in selecting hyperparameters in single-cell data analysis.

The proposed method is  evaluated extensively on  simulated datasets and multiple real-world datasets, including two benchmarking datasets from computer vision and four single-cell omics datasets (see Methods and Supplementary Table~\ref{tab: datasetoverview} for detailed description). The R package implementing our proposed method is available at the GitHub repository:
\begin{center}\url{https://github.com/zhexuandliu/MapContinuity-NE-Reliability}.
\end{center}


==> tex_files/methods_backup.tex <==
\hengheng{Is it ok to have repeated parts between Methods and the content before?}

\subsection{Verify Leave-one-out (LOO) empirically} \label{sec: method: LOO}

Our LOO claim assumes that deleting (or adding/modifying) a single input
point does not change embeddings of other points significantly. To verify LOO, we conduct the following experiment.

Let $\mX = [\vx_1,\ldots,\vx_n]^\top$ be the input data matrix, and $\mY = [\vy_1,\ldots,\vy_n]^\top$ be the matrix of embeddings. We randomly delete one point $\vx_i$ from $\mX$ to have the new input data $\mX_{-i} = [\vx_1,\ldots,\vx_{i-1},\vx_{i+1},\vx_n]^\top$. Then, with $\mY_{-i} = [\vy_1,\ldots,\vy_{i-1},\vy_{i+1},\vy_n]^\top$ as initialization, we run t-SNE algorithm to obtain the embedding of $\mX_{-i}$, denoted as $\tilde{\mY}_{-i}$. To verify LOO empirically, we keep track of the difference between $\mY_{-i}$ and $\tilde{\mY}_{-i}$:
\begin{equation}
    \epsilon_n = \frac{1}{\|\mY_{-i}\|_F}\|\mY_{-i}-\widetilde \mY_{-i}\|_F
\end{equation}
and expect $\epsilon_n$ to be small. 

The experiment is conducted with different sample size $n$ and with different types of dataset (simulated cluster data, simulated manifold data, real single-cell data, deep learning feature data). The results are reported in Appendix~\ref{sec: supp: LOO}. We observe that the approximation errors $\epsilon_n$ are small and generally decreasing in $n$, which aligns with our LOO assumption.


\subsection{Two diagnostic scores} \label{sec: appendix: diagnosis metrics}

\subsubsection{Perturbation score} \label{sec: method: perturbation score}
Given an input data matrix $\mX = [\vx_1,\ldots,\vx_n]^\top$ and its embedding matrix $\mY = [\vy_1,\ldots,\vy_n]^\top$, without loss of generality, we calculate the perturbation score for the $n$-th data point with direction as a vector $\ve$ of unit length and perturbation length $\lambda$.

Let $\widetilde{\mY} = [\widetilde{\vy}_1,\ldots,\widetilde{\vy}_{n}]^\top$ be the embedding of input data matrix $\widetilde{\mX} = [\vx_1,\ldots,\vx_n + \lambda\ve]^\top$, i.e. the input data matrix after perturbation the $n$-th data point. As stated in Section~\ref{sec:loo}, LOO assumption states that $\tilde{\vy}_i\approx\vy_i$, for $i=1,2,\ldots,n-1$ and $\tilde{\vy}_n$ is approximated as $\tilde{f}(\vx_n + \lambda\ve)$ by LOO-map $\tilde{f}(\vx) = \argmin_{\vy}L_n(\vy; \vx_n)$. We define the perturbation score for the $n$-th data point with direction $\ve$ and perturbation length $\lambda$ as $\|\tilde{f}(\vx_n + \lambda\ve) - \vy_n\|_2$. 

% if $\widetilde{\mY}$ reaches the global minimum of the original loss, $\vy = \widetilde{\vy}_n$ is the minimizer of a partial loss involving the $n$-th embedding point:
% \begin{align}
%     \widetilde{\vy}_n &= \argmin_{\vy \in \R^2} \sum_{1\le i \le n-1} \mathcal{L}\Big(w_{i,n}(\widetilde{\vy}_i, \boldsymbol{y}); v_{i,n}\big(\begin{bmatrix}\boldsymbol{X}_{-n} \\  \boldsymbol{x}_{n} + \lambda\ve \end{bmatrix}\big)\Big) 
% + Z\Big(\begin{bmatrix}\widetilde{\mY}_{-n}\\\vy\end{bmatrix}\Big) \notag\\
% & \approx \argmin_{\vy \in \R^2} \sum_{1\le i \le n-1} \mathcal{L}\Big(w_{i,n}(\vy_i, \boldsymbol{y}); v_{i,n}\big(\begin{bmatrix}\boldsymbol{X}_{-n} \\  \boldsymbol{x}_{n} + \lambda\ve \end{bmatrix}\big)\Big) 
% + Z\Big(\begin{bmatrix}\mY_{-n}\\\vy\end{bmatrix}\Big)\notag\\
% &= \argmin_{\vy \in \R^2} L_n(\vy; \vx_n + \lambda\ve)\notag
% \end{align}
% where the approximation is based on the LOO assumption that deleting (or adding/modifying) a single input point does not change embedding significantly, i.e. $\widetilde{\mY}_{-n}\approx \mY_{-n}$. Additionally, note that $\vy_n = \argmin_{\vy \in \R^2} L_n(\vy; \vx_n)$. We define the perturbation score for the $n$-th data point with direction $\ve$ and perturbation length $\lambda$ as $\|\argmin_{\vy \in \R^2} L_n(\vy; \vx_n + \lambda\ve) - \vy_n\|_2$. 

When implementing, we search the perturbation directions among the first 3 principal directions of the data $\{\ve_1, \ve_2, \ve_3\}$ and their opposites  $\{-\ve_1, -\ve_2, -\ve_3\}$, and the perturbation length $\lambda$ is specified by the user. In this way, we can further define the perturbation score of the $n$-th data point as 
\begin{equation}
    \max_{\ve\in\{\pm\ve_1, \pm\ve_2, \pm\ve_3\}}\|\tilde{f}(\vx_n + \lambda\ve) - \vy_n\|_2.
\end{equation}

In general, perturbation score is not sensitive to perturbation length. Figure~\ref{fig: appendix: sensitivity_pscore} illustrates the perturbation scores of the CIFAR10 deep learning feature data for three perturbation lengths ($\lambda \in \{1, 2, 3\}$). Points with high perturbation scores remain consistent across different perturbation lengths. In practice, we recommend that users run perturbation score on a subset of data points and test with a few different perturbation lengths. Conceptually, the perturbation score detects points that fall within a radius of $\lambda$ around the location of the OI discontinuity.

Moreover, we provide two types of approximation algorithms to accelerate the calculation of perturbation score for t-SNE along with a strategy for users to pre-screen points for which the perturbation score should be computed. 

\paragraph{Approximation method 1.} Before calculating the similarity matrix as defined in t-SNE, dimensionality reduction using PCA is required. Since each data point is perturbed multiple times in the original input space and the similarity matrix is recalculated after each perturbation, PCA must be repeated numerous times. However, for datasets of reasonable size, the effect of changing a single point on the PCA result is minimal. Approximation method 1 skips the PCA step during similarity matrix calculation, instead using the original PCA result throughout the entire process. The difference between Approximation Method 1 and the precise perturbation score is negligible for reasonably sized datasets, as perturbing a single point has only a minor impact on the overall PCA outcome.

The precision of approximation method 1 is high, making it a suitable substitute for the precise perturbation score when repeatedly performing PCA on datasets is time-consuming. As shown in Figure~\ref{fig: appendix: approx}a, perturbation score using approximation method 1 is approximately equal to precise perturbation score for almost all the points.

\paragraph{Approximation method 2.} After reducing the number of PCA computations, we can further accelerate the computation of perturbation score by approximating the similarity matrix. 

Given the input data matrix $\mX = [\vx_1,\ldots,\vx_n]^\top$ and perplexity $\mathcal{P}$, the computation of similarity scores $(v_{ij}(\mX))_{i<j}$ follows the steps below.
\begin{enumerate}
    \item Calculate the pairwise distance $d_{ij} = \|\vx_i - \vx_j\|_2$ for $i,j = 1,\ldots,n$.
    \item Find $\sigma_i$, $i=1,\ldots,n$ that satisfies
    \begin{equation}
        -\sum_{j\neq i}\frac{\exp(-d_{ij}^2/2\sigma_i^2)}{\sum_{k\neq i}\exp(-d_{ik}^2/2\sigma_i^2)}\log_2\Big(\frac{\exp(-d_{ij}^2/2\sigma_i^2)}{\sum_{k\neq i}\exp(-d_{ik}^2/2\sigma_i^2)}\Big) = \log_2(\mathcal{P}).
        \label{eqn: PMatrix solve sigma}
    \end{equation}
    \item Calculate $p_{j|i} = \frac{\exp(-d_{ij}^2/2\sigma_i^2)}{\sum_{k\neq i}\exp(-d_{ik}^2/2\sigma_i^2)}$, $i,j = 1,\ldots,n$. And 
    \begin{equation}
        v_{ij}(\mX) = \frac{p_{j|i} + p_{i|j}}{2n}.
    \end{equation}
\end{enumerate}
The main computational bottleneck is at step 2, where we conduct binary search algorithm for $n$ times to solve $\sigma_i$'s. 

Without loss of generality, we denote the input data matrix after perturbation as $\widetilde \mX = [\vx_1,\vx_2,\ldots,\widetilde\vx_n]^\top$ and the precise standard deviations solved by Equation~\ref{eqn: PMatrix solve sigma} with $\widetilde \mX$ as $\widetilde \sigma_i$, $i=1,\ldots,n$. Note that when $n$ is large, Equation~\ref{eqn: PMatrix solve sigma} still approximately holds for $i=1,\ldots,n-1s$ as only one of the $n-1$ terms in LHS changes. Therefore, $\widetilde \sigma_i \approx \sigma_i$ for $i=1,\ldots,n-1$. In this approach, using $\sigma_i$ to approximate $\widetilde\sigma_i$, $i=1,\ldots,n-1$, we only need to run the binary search algorithm once to determine $\widetilde{\sigma}_n$, and then set $\widetilde{\sigma}_i = \sigma_i$ for $i = 1, \ldots, n-1$ to compute the new approximated similarity score $(v_{ij}(\widetilde{\mX}))_{i<j}$, which significantly speeds up the calculation of the similarity matrix after perturbation. Performance-wise, it takes 21.7 seconds on a MacBook Air with Apple M2 chip to calculate the precise perturbation score of one point from a 5000 points CIFAR-10 neural network feature dataset but only takes 6.8 seconds with approximation method 2. 

The precision of approximation method 2 is also high. As shown in Figure~\ref{fig: appendix: approx}b, perturbation score using approximation method 2 is approximately equal to precise perturbation score for most of the points.

\paragraph{Pre-screening of points.} We note that high perturbation scores are often observed among points embedded at the peripheries of clusters, as points in cluster cores tend to remain within core regions of the input space, reducing their likelihood of interacting with other clusters. Therefore, calculating the perturbation score specifically for peripheral points allows us to assess both the stability of these embeddings under perturbation and the location of OI discontinuities. By leveraging the parallelism in perturbation score computation across points, pre-screening data points in this way can significantly reduce computational effort while still providing a comparable assessment of OI discontinuity locations across the entire embedding (Figure~\ref{fig: appendix: prescreen}).

We use function \texttt{dbscan} in the R package dbscan (version 1.2-0) to identify embeddings on the periphery of clusters. User can adjust the parameters in the function to adjust the pre-screened points.

\subsubsection{Singularity score}

As mentioned in Section~\ref{sec:loo}, given an input data matrix $\mX$, to find embedding matrix $\mY$, we usually need to minimize a loss function with the following form:
\begin{equation}
\mathfrak{L}(\vy_1,\ldots,\vy_n;\mX) = \sum_{1\le i<j\le n} \mathcal{L}(w_{ij}(\boldsymbol{y}_i, \boldsymbol{y}_j); v_{ij}(\mX)) + Z(\boldsymbol{Y}).
\label{eqn: loss function in method score}
\end{equation}
The embedding we obtain is the minimizer of $\mathfrak{L}(\vy_1,\ldots,\vy_n;\mX)$, denoted as $\vy_1^*,\ldots,\vy_n^*$.

We define the singularity score of the $i$-th data point as the inverse of the smallest eigenvalue of the Hessian matrix of $\mathfrak{L}$, that is
\begin{equation}
    \lambda_{\min}^{-1}(\mH_i),\quad\text{where }\left.\mH_i=\frac{\partial^2\mathfrak{L}(\vy_1,\ldots,\vy_n;\mX)}{\partial \vy_i\partial\vy_i^\top}\right|_{\vy_k = \vy_k^*,\ k = 1,\ldots,n}.
\end{equation}

Derivations of the singularity score and the rationale for its relation to the sensitivity of the embedding under infinitesimal perturbation can be found in Appendix~\ref{sec: appendix: derivation of sscore}.

\hengheng{can talk more about this. Put part of the appendix to Methods.}


% To explain the derivation of the Singularity Score, let us consider a perturbation to $\vx_i$ in the input space resulting in $\vx_i + \delta \vu$ for a given unit vector $\vu \in \R^d$. The new similarity score is denoted by $v_{ij}(\delta)$.
% Let $\vy_i(\delta) = \argmin_{\vy_i \in \R^2} \sum_{j\neq i} L(w_{ij}(\vy_i, \vy_j^*); v_{ij}(\delta))$; note $\vy_i = \vy_i(0)$. Taylor expansion on $\vy_i(\delta)$ yields (see Appendix~\ref{sec:app-todo} for details)
% \begin{equation*}
%     \vy_i(\delta) - \vy_i = -\delta \left(\frac{\partial^2 \ell_i(\vy_i) }{\partial \vy_i \partial \vy_i^\top} \right)^{-1}  \frac{\partial^2 \ell_i(\vy_i)}{\partial \vy_i \partial \vy_i^\top} \frac{\partial \vy_i}{\partial \vx_i}^\top \vu + o(\delta).
% \end{equation*}
% The matrix inversion is likely the source of observed discontinuity. The smallest eigen value
%     \begin{equation*}
%         \mathrm{score}_i = \lambda^{-1}_{\min}\left(\frac{\partial^2 \ell_i(\vy_i) }{\partial \vy_i \partial \vy_i^\top} \right)
%     \end{equation*}
% is used as our measure of embedding stability. 


\subsection{Implementation of t-SNE}
We used the function \texttt{Rtsne()} in the R package Rtsne (version 0.17) to perform the t-SNE algorithm. We used "\texttt{theta = 0}" to perform exact t-SNE. We also adjusted the code in Rtsne to access the similarity score $p_{ij}$ in the original space. The adjusted function \texttt{Rtsne()} can be found in \url{https://github.com/zhexuandliu/RtsneWithP}.

\subsection{CIFAR-10 data}
We performed forward pass in pretrained ResNet-18 model \cite{ResNet18_CIFAR10} on CIFAR-10 test dataset to extract features of size 512. We also performed forward pass in the same model on Describable Textures Dataset (DTD) dataset to serve as our out-of-distribution data in Section~\ref{sec:OOD Detection}. We randomly subsample the datasets for the time and cost of computation. In Section~\ref{sec:intro}, we use a subset of size $5000$ for CIFAR-10 deep learning feature data. In Section~\ref{sec:OOD Detection}, we use a subset of size $2000$ for CIFAR-10 deep learning feature data and a subset of size $1000$ for DTD deep learning feature data. The preprocessed data are provided in the Source Data file.

\subsection{Mouse brain ATAC-seq data}
Single-cell ATAC-seq dataset of mouse brain cells provided by 10x Genomics \cite{10XGenoMouseBrainATAC} is preprocessed, normalized by R package Seurat (version 5.0.3). We applied the function "\texttt{FindVariableFeatures()}" in Seurat to identify 1000 most variable genes for 3618 samples. The preprocessed data are provided in the Source Data file.

\subsection{Mouse embryonic stem cell differentiation data}
The RNA-seq data of mouse embryonic stem cells (mESCs) undergoing differentiation \cite{HayashiData} is preprocessed, normalized by R package Seurat (version 5.0.3). We also used Seurat to identify 2000 most variable genes for all 421 samples. The preprocessed data are provided in the Source Data file.

==> tex_files/related-work.tex <==
\Rong{we can shorten and move this part to the Introduction section.}

% Stochastic neighbor embedding methods such as t-SNE and UMAP have become the de facto standard for visualizing high-dimensional data, especially in the context of single-cell RNA sequencing, image embeddings, and other forms of biomedical data. However, recent research has shown that SNE methods can often produce misleading results. Spurious clusters can emerge, and global structure is often not well-preserved in these embeddings \cite{PaCMAP}. Significant distortions in both local and global preservation are introduced by such dimensionality reduction methods \cite{ChariSpeciousArt2023}. Additionally, the embedding is sensitive to the choice of optimization approaches \cite{YangOptimizationTSNE2015}, random seeds for initialization \cite{KobakInitializationImportantForTSNEUMAP2019}, and tuning hyperparameters \cite{KobakInitializationImportantForTSNEUMAP2019,Ma2022theoreticalfoundationoft-SNE}.

% To address these issues, recent research has developed guidelines and methods for optimizing hyperparameter selection to achieve more accurate and reliable embeddings \cite{ChariSpeciousArt2023, wattenberg2016how, kobak2019art, BelkinaAutoOptParaTSNE2019,scDEED2023}. Metrics like KL-divergence between kernels and the correlation of nearest-neighbor distances in both input and embedding spaces have been proposed to identify embeddings with severe neighborhood distortion \cite{EMBEDR, scDEED2023}. These approaches help in identifying and mitigating the artifacts that can arise in embeddings.

% In this paper, we recognize that these issues, such as distortions and sensitivity to parameters, stem from an inherent discontinuity in the embedding map. While efforts have been made to learn the embedding map using neural networks \cite{vandermaatenParaTSNE2009}, the mapping is still not explicitly defined in a parametric form, making it challenging to study. Indeed, only the existence and uniqueness of such an embedding map have been proven \cite{auffinger2023equilibriumdistributionstdistributedstochastic}, and the approach for understanding the properties of the embedding map remains underdeveloped.

% By introducing LOO, we provide a novel approach to examine the embedding map locally rather than analyzing it globally. The decoupling of the loss function allows us to better understand the behavior of the embedding map and identify OI and FI discontinuity that may lead to misleading visualizations. Our work offers new insights into the nature of embedding maps, which can enhance the reliability of stochastic neighbor embedding methods.

==> tex_files/to-do.tex <==
\section*{Discussion lists}

\TODO{Change from ``stochastic neighbor embedding methods'' to ``neighbor embedding methods'' in title. Please check that we make all necessary replacements throughout the paper.}

\hengheng{I think we should say neighbor embedding methods. Need to change the title then?

As in https://openreview.net/pdf?id=tNXumks8yHv (we should cite this btw. This paper show that SNE, t-SNE, LargeVis and UMAP are all instances of graph coupling and characterized by different choices of prior for discrete latent structuring graphs.)

and https://proceedings.mlr.press/v202/peltonen23a/peltonen23a.pdf, I quote 'These will be referred to as SNE-like or neighbor embedding methods in what follows'. Meanwhile, stochastic neighbor embedding is typically referred to as SNE method \cite{HintonSNE2002}.}

\hengheng{I put the citation about NE methods are graph coupling, and minimum distortion embedding here. Do we need to talk more at this point?} \TODO{I think it is fine.}

~ Section 2\\

\TODO{Do we want to emphasize the difference between the two scores? One is a more global property affecting a larger area, another is a local property.} \TODO{There is a difference between adding a new point vs.~perturbing a point. Do we want to emphasize it here or later? I prefer later.} \hengheng{I think later is better. When bringing out point-wise score, we can say $\vy_n$ is the mapping of $\mX_n$ induced by the LOO-map of $\mX_{-n}$ and $\mY_{-n}$ (as $\mY_{-n}$ is an embedding of $\mX_{-n}$ by LOO-assumption), thus softening the difference between adding and deleting one point.}


~ Section 2.2\\
\hengheng{rerun the experiment}
%\TODO{In paragraph ``LOO loss function and LOO-map'', we can cite some additional classical papers on LOO. I believe Grace Wahba has some? I also have some theoretical papers.}

~ Section 2.5 \\
\TODO{DO we need more statistics and detailed quantitative evaluation? It seems that many papers analyze single-cell data in great detail. Perhaps it is sufficient now, since one of our main contributions is conceptual rather than factual.}

~ Section 3

\TODO{Limitation and future work: (1) other distortion factors not covered, we may improve t-SNE by combining parametric embedding with t-SNE to improve both interpretability and faithfulness (2) consider scaling up the method to large-scale datasets in future work (3) a mathematical framework, nonparametric approach?.} 
